UnQovering Stereotyping Biases via Underspecified Questions

While language embeddings have been shown to have stereotyping biases, how these biases affect downstream question answering (QA) models remains unexplored. We present UNQOVER, a general framework to probe and quantify biases through underspecified questions. We show that a naive use of model scores can lead to incorrect bias estimates due to two forms of reasoning errors: positional dependence and question independence. We design a formalism that isolates the aforementioned errors. As case studies, we use this metric to analyze four important classes of stereotypes: gender, nationality, ethnicity, and religion. We probe five transformer-based QA models trained on two QA datasets, along with their underlying language models. Our broad study reveals that (1) all these models, with and without fine-tuning, have notable stereotyping biases in these classes; (2) larger models often have higher bias; and (3) the effect of fine-tuning on bias varies strongly with the dataset and the model size.

==> [EMNLP'20] Unqovering Stereotypical Biases via Underspecified Questions/macros.tex <==
\newcommand{\tao}[1]{{\small \color{red} [TL: #1]}}
\newcommand{\ashish}[1]{{\small \color{violet} [AS: #1]}}
\newcommand{\tushar}[1]{{\small \color{orange} [TK: #1]}}
\newcommand{\daniel}[1]{{\small \color{blue} [DK: #1]}}
\newcommand{\vs}[1]{{\small \color{darkgreen} [VS: #1]}}
\newcommand{\todo}[1]{{\small \color{purple} [TODO: #1]}}

\usepackage{subfigure}

% \newcommand{\tao}[1]{}
% \newcommand{\ashish}[1]{}
% \newcommand{\tushar}[1]{}
% \newcommand{\daniel}[1]{}
% \newcommand{\vivek}[1]{}
% \newcommand{\todo}[1]{}

% \newcommand{\name}{\textsc{Underspecied}}
% \newcommand{\name}{\textsc{Undie}}
\newcommand{\name}{\textsc{UnQover}\xspace}

\definecolor{purple}{rgb}{0.5,0,1}
\definecolor{dcyan}{rgb}{0.2,0.6,0.5}
% \definecolor{darkgreen}{rgb}{0,200,0}
\definecolor{light-gray}{gray}{0.95} % used in table
\definecolor{darkgreen}{RGB}{0,140,0}
\definecolor{darkred}{RGB}{200,0,0}
\definecolor{lightgreen}{RGB}{189,252,192}
\definecolor{lightred}{RGB}{255,205,212}
\definecolor{lightyellow}{RGB}{255,240,160}
\definecolor{lightblue}{RGB}{195,221,255}
\definecolor{lightpurple}{RGB}{232,209,255}



\newcommand{\slot}[1]{[\textit{#1}]}
\newcommand{\sfiller}[1]{{\color{blue} \textit{#1}}}
\newcommand{\afiller}[1]{{\color{red} \textit{#1}}}
\newcommand{\prob}[1]{\mathbb{P}\left(#1\right)}
\newcommand{\score}[1]{\mathbb{S}\left(#1\right)}
\newcommand{\bias}[1]{\mathbb{B}\left(#1\right)}
\newcommand{\unqover}[1]{\mathbb{C}\left(#1\right)}

\newcommand{\bertbase}{BERT$_{\textrm{B}}$\xspace}
\newcommand{\bertlarge}{BERT$_{\textrm{L}}$\xspace}
\newcommand{\bertboth}{BERT$_{\textrm{B/L}}$\xspace}
\newcommand{\robertabase}{RoBERTa$_{\textrm{B}}$\xspace}
\newcommand{\robertalarge}{RoBERTa$_{\textrm{L}}$\xspace}
\newcommand{\robertaboth}{RoBERTa$_{\textrm{B/L}}$\xspace}
\newcommand{\distilbert}{BERT$_{\textrm{Dist}}$\xspace}

\newcommand{\egbox}[1]{
\smallskip
\noindent
\fbox{
        \parbox{0.95\linewidth}{
        \vspace{0.5ex}#1\vspace{0.5ex}}
      }
\smallskip
}

\newcommand{\egboxwide}[1]{
\smallskip
\noindent
\fbox{
        \parbox{0.97\linewidth}{
        \vspace{0.5ex}#1\vspace{0.5ex}}
      }
\smallskip
}

% \newtheorem{theorem}{Theorem}[section]
% \newtheorem{corollary}{Corollary}[theorem]
% \newtheorem{lemma}[theorem]{Lemma}

\newtheorem{theorem}{Theorem}
\newtheorem{corollary}{Corollary}
\newtheorem{lemma}{Lemma}
\newtheorem{prop}{Proposition}


==> [EMNLP'20] Unqovering Stereotypical Biases via Underspecified Questions/old_equations_may20.tex <==
% \section{Reasoning Errors and Biases}
\section{Reasoning Errors of Question Answering Models and their Biases}
\label{sec:unintended_bias}
Before we go into the details of how we use our examples to detect biases, lets first consider \emph{what we can observe} as the output of our model and what \emph{we want to measure}. Given our generated examples and a QA model, we can measure the score assigned to a subject $x_1$ for the question based on $a$, represented as $\prob{x_1|\tau(x_1, x_2, a)}$ where $\tau(x_1, x_2, a)$ captures the (paragraph, question) pair generated by grounding our template $\tau$. For a QA model, these \daniel{simply} are \daniel{\sout{naturally}} probabilities of the span $x_1$ and $x_2$. 
\daniel{from this phrasing, is it clear that $\prob{x_1} + \prob{x_2} \neq 1$?}
For masked LM, we can use the probabilities for these subject tokens (assuming single-token subjects). However, what we want to measure is the stereotypical bias associated with $x_1$ compared to $x_2$ for $a$, represented as $\score{x_1| \{x_1, x_2, a\}}$.
%Note that the stereotypical bias score does \emph{not} depend on how the subjects and attributes are grounded by our template. \daniel{I don't understand this. Clarify this?}\tushar{actually this is not important in this formulation, so okay to drop.}

\daniel{
In $\score{x_1| \{x_1, x_2, a\}}$ notation, the use of set notation makes it seem like the ordering of $x_1, x_2, a$ does not matter, which is not the case. 
}

A natural approach to measure the bias, $\score{x_1| \{x_1, x_2, a\}} - \score{x_2| \{x_1, x_2, a\}}$ would be by directly comparing these predicted probabilities associated with the two subjects~\cite{de2019bias}, i.e., the bias of the model towards \slot{$x_1$} for activity \slot{$a$} could be measured as:
{
% \small
%\begin{equation}
\begin{align}
\score{x_1| \{x_1, x_2, a\}} - \score{x_2| \{x_1, x_2, a\}} = \nonumber\\
  \prob{x_1| \tau(x_1, x_2, a)} - \prob{x_2| \tau(x_1, x_2, a)}
\label{eqn:bias_score}
\end{align}
%\end{equation}
}
However, models sometimes focus on artifacts in the input leading to inconsistent behaviors. For example, $\score{x_1| \{x_1, x_2, a\}}$ does not depend on the ordering of $x_1$ and $x_2$, i.e.  $\score{x_1| \{x_1, x_2, a\}}=\score{x_1| \{x_2, x_1, a\}}$, but this is not the case with a RoBERTa SQuAD model:
%\emph{[An example with extreme probabilities and inconsistent predictions]}
\egbox{
    
    {\small Paragraph: The person over the swing is \sfiller{Justin}. Sitting by the side is \sfiller{Alice}.}\\
    {\small Question: Who \afiller{was a bodyguard}? }\\ 
    \text{   } {\small $\prob{\sfiller{Alice}}\texttt{=}0.77$ \hspace{2ex} $\prob{\sfiller{Justin}}\texttt{=}0.21$.} \\
    \\
    {\small Paragraph: The person over the swing is \sfiller{Alice}. Sitting by the side is \sfiller{Justin}.}\\
    {\small Question: Who \afiller{was a bodyguard}? }\\ 
    \text{   } {\small $\prob{\sfiller{Alice}}\texttt{=}0.03$ \hspace{2ex} $\prob{\sfiller{Justin}}\texttt{=}0.96$.}
    }
where predictions are completely changed by just swapping the subjects positions, even though the information in the context is effectively the same.
%\tushar{Can we change the example with a more symmetric context? Arguably bodyguards are never the ones on swings :)}



%In this paper, we aim to measure stereotypical biases via underspecified questions. That is, with both subjects are equally justifiable for a question, model should predict fair distribution over them. Unfair predictions can be attributed to biases, known or unknown, and reasoning errors. When measuring stereotypical biases, we expect a metric to be as robust as possible against errors and variances such that there is no false positive.

%In this section, we present our discoveries on two major categories of reasoning errors that exist in both QA and pre-trained language models: \textbf{position inconsistency} and \textbf{negation inconsistency}. We argue that a robust evaluation has to peel off the effect of such reasoning errors, otherwise one might end up with contradicting observations.

Furthermore, models might not always capture what the question is intended to ask:
%While our bias score is position invariant, it should be highly dependent on the attribute in the question. However, models may not always capture the question accurately, e.g., the RoBERTa SQuAD model has roughly the same scores for two questions with exactly opposite meaning!
%consider the example predictions from a RoBERTa SQuAD model:
%\emph{[An example with extreme probabilities and inconsistent predictions]}
\egbox{
    {\small Paragraph: The person over the swing is \sfiller{Justin}. Sitting by the side is \sfiller{Alice}.}\\
    {\small Question: Who \afiller{was a bodyguard}? }\\ 
    \text{   } {\small $\prob{\sfiller{Alice}}\texttt{=}0.77$ \hspace{2ex} $\prob{\sfiller{Justin}}\texttt{=}0.21$.} \\
    {\small Question: Who \afiller{can never be a bodyguard}?} \\
    \text{   } {\small $\prob{\sfiller{Alice}}\texttt{=}0.87$ \hspace{2ex} $\prob{\sfiller{Justin}}\texttt{=}0.10$.}
}

\emph{Given these reasoning errors\footnote{We call them reasoning errors since a robust model should not be affected by such meaning invariant changes (and should be affected by the change in question meaning).}, how can we accurately capture the stereotypical biases of QA models?} We will show how these issues can be isolated to reveal the true stereotypical bias in the model. 

\subsection{Decomposing Reasoning Errors and Biases}
While the stereotypical bias $\score{x_1| \{x_1, x_2, a\}}$ is based on all of its inputs, the model scores could be affected by artifacts based on partial inputs. We capture this as a linear combination of the bias term with all possible partial interactions that are not indicative of this bias:
\begin{align}
    %\forall \tau, \prob{x_1| \tau(x_1, x_2, a)} =  \score{x_1| \{x_1, x_2, a\}} + \nonumber\\
    %f(x_1, x_2, \tau) + g(\{x_1, x_2\}, a) \label{eqn:components}
    \forall \tau, &\; \prob{x_1| \tau(x_1, x_2, a)} =  \score{x_1| \{x_1, x_2, a\}} + \nonumber\\
    & f(x_1| x_2, \tau) + g(x_1 |x_2, a) \label{eqn:components}
\end{align}
%We basically assume that the model's score is a linear combination of a robust score based on all the inputs (i.e. the bias) and all possible partial interactions within $\{x_1, x_2, a\}$ that would not capture the bias.
where the first component $f(x_1 | x_2, \tau)$ captures the models' preference purely based on the paragraph irrespective of the attribute; the second component $g(x_1 | x_2, a)$ captures the model's preference purely based on lexical cues in the attribute irrespective of the subject ordering and sentence structure in $\tau$.\tushar{We shouldn't have "a" in g. The point is that g is the factor that does not depend on a. So it would stay the same for both a and $\bar{a}$. I see the value of $x_1|x_2$ in g as it makes it clear that the bias is towards $x_1$ but it also makes it seem order-dependent.}
%Note that model's decisions to choose any subject purely based on the question would still fall under the umbrella of bias. For simplicity, we ignore terms purely based on $a$ as they would appear in $\prob{x_2| \tau(x_1, x_2, a)}$ too and cancel each other out. 
%Henceforth, we will only model $g(x_1)$ and assume $h(x_2)$ would be captured by $\prob{x_2| \tau(x_1, x_2, a)}$.

Our goal here is to isolate the components $f$ and $g$ for the a given template $\tau$. To isolate $f$, we will use subject-symmetric examples $\tau(x_1, x_2, a)$ and $\tau(x_2, x_1, a)$ where the only variant for the model to make different predictions would be the subject position. We will refer this to \emph{positional artifact} in Sec~\ref{subsec:position_bias}.
For component $g$, we will use polarized attributes\tushar{What are polarized attributes?} where models rely on lexical cues in the attribute to make predictions. We will refer this to \emph{attributive artifact} in Sec~\ref{subsec:preference_bias}.


%The first term:  $f(x_1, x_2, \tau)$ captures the score purely based on the paragraph. For symmetric templates, the information captured by $\tau(x_1, x_2, a)$ should be exactly same as $\tau(x_2, x_1, a)$. \tao{dont want to say exactly.} So the only phenomenon that the model relies on to make different predictions for $\tau(x_1, x_2, a)$ vs $\tau(x_2, x_1, a)$ would be the position of these subjects. Note that even if the template is not symmetric, our solution to factor out the term $f(x_1, x_2, \tau)$ would correct any position-specific bias introduced by our templates. \tao{the last sent is too detailed.}


%The second term: $g({x_1, x_2}, \tau)$ captures the model's relative preference toward a particular subject irrespective of order and the attribute in the question. It may also be relying on lexical cues from the template, but importantly does not rely on the input attribute. The influence of this term can be seen in the example above, where changing the question had minimal effect due to the dominant effect of this score. 

Since these are the only possible terms that do not capture bias, if we factor these terms out, we will be left with only the sterotypical bias of the model. We will focus on isolating these reasoning errors individually first and then combine them to derive our final score.

%So can we say the model is actually fair because some reasoning errors overwrite stereotypical biases (if there is any)? We will show the asnwer is \emph{no}. After peeling off errors in model predictions, stereotypical biases are revealed.


\subsection{Positional Artifacts($\mu$)}
\label{subsec:position_bias}
As shown above, flipping subject positions would change model predictions.
But this shouldn't change the bias score.
By measuring this shift in model scores between the two orderings, we can measure this error:
%\tao{Doing simplification}
%As we show above, certain models have an implicit tendency to pick one subject over another purely based on its position in text. In such a case, flipping the subject positions would change the model predictions, but shouldn't change the bias score.  
%In such a case, flipping the answer positions would also flip model predictions. This \emph{flip} in model predictions can be measured by comparing the shift in probability between the two subject orderings. Specifically we can measure this type of error on the \emph{second} subject as:
{
\begin{align*}
    \mu(x_1, x_2, a) = \prob{x_1| \bar{\tau}(a)} \texttt{-} \prob{x_1| \tau(a)}
\end{align*}
}
where $\tau(a)$ denotes the subject-instantiated example $\tau(x_1, x_2, a)$ and the flipped version $\bar{\tau}(a)=\tau(x_2,x_1,a)$\footnote{We will assume there is only one template $\tau$ to simplify notation. In practice, we use multiple templates.}.
Given our definition in Eq~\ref{eqn:components}, 
%$\prob{x_1| \tau(x_1, x_2, a)} =  \score{x_1| \{x_1, x_2, a\}} + f(x_1, x_2, \tau)$, 
this score captures the relative bias between the two positions, i.e.
\begin{align*}
        \mu(x_1, x_2, a) = f(x_1 | x_2, \tau) - f(x_1 | x_2, \bar{\tau})
\end{align*}


We can also measure this value for our entire dataset by aggregating this value across all the examples, i.e.,
{
\begin{equation}
    \label{eq:pos_score}
    \mu = \frac{\sum_{
        \substack{
            x_1\in X_1 \\ 
            x_2\in X_2 \\ 
            a \in A
        }
    } \mu(x_1, x_2, a) }{|X_1| \times |X_2|\times|A|},
\end{equation}
}
where $X_1$ and $X_2$ are the set of subjects and $A$ are the set of attributes. $\mu$ falls in range $[-1,+1]$ and would be zero for a model with no position bias. 

\paragraph{Isolating Positional Artifacts.} 
While we can not directly measure $f$, by averaging the model's scores for both positions, we can factor them out in our comparative bias computation, i.e., we compute the position-invariant score for $x_1$ as
%When measuring the true stereotypical bias, we need to factor out this inconsistency. To do so, we include both orderings of subjects in our example and average the two probabilities to get the model's preference towards a particular subject. The position-corrected score for subject $x_1$ would be:
%We will introduce our metric in Section~\ref{sec:metric}
% \tushar{This is different though, right? It is talking about what it would mean to only isolate position bias and I am hoping gives intuition about the final metric.}

\begin{align*}
  &s_{\mu}(x_1| a) \texttt{=} \frac{1}{2}\Big[\prob{x_1| \tau(a)} \texttt{+}  \prob{x_1| \bar{\tau}(a)}\Big] \\
   &\hspace{2ex}\texttt{=}\score{x_1| \{x_1, x_2, a\}} \texttt{+} g(x_1|x_2,a) \texttt{+} \\
   & \hspace{3ex} \frac{1}{2}\Big[ f(x_1|x_2,\tau) \texttt{+} f(x_1|x_2,\bar{\tau})\Big]
  %=& \score{x_1| \{x_1, x_2, a\}} + \frac{1}{2}\Big[ f(\tau) + f(\bar{\tau})\Big]
\end{align*}
In the running example, when the activity $a$=\afiller{was a bodyguard}, we have $s_\mu(\sfiller{Alice})=0.4$ and $s_\mu(\sfiller{Justin})=0.59$.

%\tao{We are not done yet. Too early to jump to the below conclusion.}
%i.e. the model was actually biased towards \sfiller{Justin} being the \afiller{bodyguard}. Also note that the latter term would be exactly same for $\score{x_2| \{x_1, x_2, a\}}$ and so the final comparative bias based on this score would capture the true stereotypical bias:
%\begin{align*}
%&s_{\mu}(x_1| \tau(a))  -  s_{\mu}(x_2| \tau(a)) = \\
%& \hspace{1ex} \score{x_1| \{x_1, x_2, a\}}  - \score{x_2| \{x_1, x_2, a\}} + \\
%& \hspace{1ex} g(x_1|x_2,a) - g(x_2|x_1,a)
%\end{align*}
%where we assume position has a linear component in model predictions.



%Similar score can be computed for \slot{$x_2$} and then compared to $ \text{score}(x_1| x_2, a)$ to get the model's bias. Note that for a model with no position bias, i.e $\mu_2(x_1, x_2, a) = 0$, these two probabilities would be exactly same and map to the model's predicted probability.
%In our underspecified setting, we consider position bias as how much a subject's position is preferred over the other position. We measure it by the averaged winning score of the first subject over the second subject over all examples and questions. We denote it by $\mu(1st)$, and $\mu(2nd)=-\mu(1st)$.

%\tushar{TODO: Add simple example to map this equation to a real example}

\subsection{Attributive Artifacts ($\nu$)}
\label{subsec:preference_bias}
%But is it true even if the question is negated?
% We have seen that, in the above example, sometimes models seem do not understand the question.
%This kind of inconsistency is very hard to detect as it would appear very similar to the stereotypical bias in the model. For example, if the model is biased towards a particular subject for all activities in our set, it would also appear as a preference bias.
%To measure such errors, we need to introduce alternate activities that would change the prediction of the stereotypical bias model. but not the model with preference bias. Specifically, for every activity in our set $a$, we introduce a negated activity $\bar{a}$ such that a stereo-typical model, that chooses $x_1$ as the answer for $a$, would \emph{not} choose it be the answer for $\bar{a}$, i.e. anti-stereotypical. For example, for the activity: $a$=\afiller{is a country full of poor people}, we create a negated activity: $\bar{a}$ = \afiller{is a country full of rich people}. 
Unlike positional artifact, we expect the bias score to change with the attribute. But as we observe, this may not be the case in our QA models. So to measure this error, we need to introduce an attribute that should, by design, change the model prediction and then measure the model's invariance.

%Specifically, we use a negated attribute $\bar{a}$ for each $a$ such that a stereotypical model, that chooses $x_1$ as the answer for $a$, would ideally not choose it for $\bar{a}$.

For subject $x_1$, we can measure this error based on the change in probabilities over the polarized pair $(a,\bar{a})$:
%At each instance level, we can compare the scores across two polarized activities: $P(x_1| \tau(x_1, x_2, a))$ and $P(x_1| \tau(x_1, x_2, \bar{a}))$ which when aggregated across the examples gives us the preference bias of the model:
{
\begin{align}
    \nu(x_1, x_2, a) & = 1 \texttt{-} \Big| \prob{x_1| \tau(a)} \texttt{-} \prob{x_1| \tau(\bar{a})} \Big|  \nonumber 
\end{align}

\begin{align}
    \nu = \frac{\sum_{x_1 \in X_1, x_2 \in X, a \in A} \nu(x_1, x_2, a)}{|{X_1}|\times|{X_2}|\times|A|},
        \label{eq:pref_score}
\end{align}
}
where $\tau(\bar{a})=\tau(x_1,x_2,\bar{a})$. 
%Note that a model, that blindly prefers a particular answer irrespective of the activity, would not have much change in predictions.
Note that when the model ignores the semantics of attribute $a$, it would have $g(x_1| x_2, a)=g(x_1|x_2,\bar{a})$ resulting in $\nu=1$, whereas any difference in probabilities would reduce this score.
% Specifically given $\prob{x_1| \tau(x_1, x_2, a)} =  \score{x_1| \{x_1, x_2, a\}} + g(\{x_1, x_2\}, \tau)$, this term captures $\nu(x_1, x_2, a) = 1 - |\score{x_1| \{x_1, x_2, a\}} - \score{x_1| \{x_1, x_2, \bar{a}\}}|$.
%Note that lack of stereotype is also a form of attribute invariance, which would appear as $\nu=0$. 
%\tushar{This might be a better metric: higher implies more bias and change in signs doesn't cancel things out.} 
%\tushar{Both this metric and our previous metric has another problem: Lack of stereotypical bias would appear as preference bias.}

\paragraph{Isolating Attribute Invariance} To factor out this error, we adopt a similar approach as in Section~\ref{subsec:position_bias}, i.e. to include both polarized activities in our example. But unlike positional artifacts, we want to measure the relative change, captured by the difference between the two scores:
%Our metric in Section~\ref{sec:metric} will score each example based on the relative preference of an activity over its negated counterpart.
\begin{align*}
  & s_{\nu}(x_1|\tau(a)) \texttt{=} \frac{1}{2}\Big[\prob{x_1| \tau(a)} \texttt{-} \prob{x_1| \tau(\bar{a})}\Big] \\
  %& \hspace{2ex} \textt{=} 
\end{align*}
In the running example, we have $s_\nu(\sfiller{Alice})=-0.05$ and $s_\nu(\sfiller{Justin})=0.05$.

This metric would automatically factor out the attribute invariant term: $g(\{x_1, x_2\}, \tau)$. Moreover, if we assume that $\score{x_1| \{x_1, x_2, \bar{a}\}}$ = $C - \score{x_1| \{x_1, x_2, a\}}$, for some constant C, this metric will give us the exact bias score shifted by a constant term:
\begin{align}
    s_{\nu}(x_1|\tau(a)) =  &\frac{1}{2}\Big[\score{x_1| \{x_1, x_2, a\}} - \nonumber\\
    & \hspace{0.5cm} \score{x_1| \{x_1, x_2, \bar{a}\}}\Big] \nonumber\\
     = &\score{x_1| \{x_1, x_2, a\}} - \frac{C}{2}
     \label{eq:pref_fix}
\end{align}
and the difference $s_{\nu}(x_1|\tau(a))-s_{\nu}(x_2|\tau(a))$ exactly captures the comparative stereotypical bias.
%And the difference $s_{\nu}(x_1|\tau(a)) & - s_{\nu}(x_2|\tau(a))$ would accurately capture the true score:
 %    \score{x_1| \{x_1, x_2, a\}}& - \score{x_2| \{x_1, x_2, a\}}$
In the next section, we will present our final metric to compute stereotypical bias based on these two metrics.
%\tushar{TODO: Add the underlying linear combination assumption. Also add the caveat for what happens when $a=\bar{a}$ for a model}

%\tushar{Should we halve this?}
%In such a case, flipping the order of the subjects would also flip the answer selected by our model. This \emph{flip} in model predictions can be measured by comparing the shift in probability between the two subject orderings. Specifically we can measure the bias towards the second subject as, i.e.
% At instance level, we consider preference bias as how much the probability changes on a particular subject when the question activity is negated. We measure this in absolute scale:
% {\small
% \begin{align}
%     \nu(t, \alpha) =& \frac{1}{2} \big(| P(x_1|t,a)-P(x_1|t,\bar{a}) | \nonumber \\
%     & +|P(x_2|t,a) - P(x_2|t,\bar{a})| \big)
%     \label{eq:pos_score}
% \end{align}
% }
% and at dataset level, we take the average over example $t$'s and activity pair $\alpha$'s. Ideally, a model predicts drastically different probabilities on the negated activity pair $\alpha$, such that $\nu=1$.

\section{Uncovering Stereotypical Biases} \label{sec:metric}
In this section, we will combine our mitigation tactics to define our final sterotypical bias score for any example. We then present two metrics to aggregate these scores across examples.

\subsection{Example Bias Score}
Lets consider Equation~\ref{eqn:components} with both the confounding factors. While each of our individual proposed scores only handle one of these factors, a simple combination of these scores cancel both of the factors out. Specifically, a simple combination of ideas from $s_\mu$ and $s_\nu$ leads to a metric that captures only the stereotypical bias score:
{\small
\begin{align}
    \gamma(x_1| x_1, x_2, a) \texttt{=} & \frac{1}{2} \Big[ s_\mu(x_1|\tau(a)) \texttt{-} s_\mu(x_1|\tau(\bar{a})) \nonumber\\
    & \texttt{-} \big[ s_\mu(x_2|\tau(a)) \texttt{-} s_\mu(x_2|\tau(\bar{a})) \big] \Big] \nonumber
\end{align}}
where $s_\mu(x_1|\tau(a)) \texttt{-} s_\mu(x_1|\tau(\bar{a}))$ captures the position-adjusted (within $s_\mu$) and attribute-adjusted (through the difference between $a$ and $\bar{a}$) score for $x_1$. The first half can be shown to simplify to the exact same term as Equation~\ref{eq:pref_fix}
{\small
\begin{align}
   & s_\mu(x_1|\tau(a)) \texttt{-} s_\mu(x_1|\tau(\bar{a}) \nonumber \\
   &=  \score{x_1| \{x_1, x_2, a\}} + \frac{1}{2}\big[ f(\tau) + f(\bar{\tau})\big] + g(\{x_1, x_2\}, \tau) \nonumber\\
   & -  \Big[\score{x_1| \{x_1, x_2, \bar{a}\}} + \frac{1}{2}\big[ f(\tau) + f(\bar{\tau})\big] + g(\{x_1, x_2\}, \tau)\Big] \nonumber\\
   & =  \score{x_1| \{x_1, x_2, a\}} - C/2 \nonumber
\end{align}}
We can prove a similar result for the second half leading to the difference between the terms capturing the true sterotypical bias:
{\small
\begin{align*}
    \gamma(x_1| x_1, x_2, a) \texttt{=} \score{x_1| \{x_1, x_2, a\}} - \score{x_2| \{x_1, x_2, a\}}
\end{align*}
}
An alternate equivalent formulation can also be similarly proven to capture the true bias:
{\small
\begin{align}
    \gamma(x_1| x_1, x_2, a) \texttt{=} & \frac{1}{2} \Big[ s_\nu(x_1|\tau(a)) \textt{+} s_\nu(x_1|\bar{\tau}(a)) \nonumber\\
    & \texttt{-} \big[s_\nu(x_2|\tau(a)) \textt{+} s_\nu(x_2|\bar{\tau}(a)) \big] \Big]
\end{align}}
where  $s_\nu(x_1|\tau(a)) \texttt{+} s_\nu(x_1|\bar{\tau}(a)))$ captures the position-adjusted (through the averaging across $\tau$ and $\bar{\tau}$) and attribute-adjusted (within $s_\mu$) score for $x_1$
\tushar{Tao: Does the above look correct?}


Consider the four example questions created through a single template in Figure~\ref{fig:example}. In essence, we first compute the position adjusted score by summing the scores for the two different orders in each row. We then subtract the bottom scores from the top to get the true stereotypical score for each $x_1$ and $x_2$. \tushar{Very hand-way. should we add the exact computation?}

We next present our two aggregate metrics that capture the models bias towards \textbf{one} subject relative to all others. 

\subsection{Subject Bias Score}

% By directly comparing two subjects in our examples, the degree of bias is naturally reflect by how much a subject is preferred over another. We argue that such comparison must be made after peeling off the effect of position and preference inconsistencies. For how much subject $x_1$ wins over $x_2$:

% {\small
% \begin{align}
%     & \gamma(x_1| x_1, x_2, a) \\ 
%     & \texttt{=} \frac{1}{2} \big[ s_\mu(x_1|\tau(a)) \texttt{-} s_\mu(x_1|\tau(\bar{a})) \texttt{+} s_\mu(x_2|\tau(\bar{a})) \texttt{-} s_\mu(x_2|\tau(a)) \big] \nonumber \\
%     & \texttt{=} \frac{1}{2} \big[ s_\nu(x_1|\tau(a)) \textt{+} s_\nu(x_1|\bar{\tau}(a)) \texttt{-} s_\nu(x_2|\tau(a)) \textt{-} s_\nu(x_2|\bar{\tau}(a)) \big] \nonumber
% \end{align}}
% \daniel{in the 2nd line, the bars should on on a's not tau's?}
% \daniel{also, I am not sure if you actually need the 2nd line}
% That is, the probability difference $\gamma$ is computed by subtracting the position-independent and negation-independent score of $x_2$ from that of $x_1$.


\begin{figure*}
    \centering
    % you can update the figure here: https://www.draw.io/#G1I9uZ2Ts7s6ygpOoqUdjbzQGA88al4-Q- 
    \includegraphics[scale=0.71]{figures/example-2.pdf}
    \caption{TODO}
    \label{fig:example}
\end{figure*}

% \tushar{TODO An example with all four instantiations of one template}
% \daniel{added an example to figure: Figure~\ref{fig:example}; some numbers are missing but see if the general structure looks good. }
%Our per-example stereotypical bias score $\gamma$ represents how probabilities are massed towards one subject over the other. 
Since these measurements can be volatile per-example\tushar{This seems a bit backward. We designed our approach with this issue in mind and not just designing the solution now. Rather we should say that we use our per-example score to capture the subject-level bias via aggregation.}, we aggregate them across examples to capture the model bias on subject $x_1$: 

{
\begin{align}
    & \gamma(x_1) = \frac{\displaystyle \sum_{\substack{\tau \in T, a\in A \\ x_2 \in X}} \gamma(x_1| x_1, x_2, a) }{|A|\times|T|\times|x_2|}
\end{align}
\daniel{should we use $\tau$ somewhere inside the parenthesis of $\gamma$?}
}
where $X$ denotes the set of subjects, $T$ the set of templates, $A$ the set of activities.
Ideally, a fair model would have $\gamma=0$. Having positive $\gamma$ indicates subject $x_1$ is biased towards the activity, and negative score represents the subject is biased away from the activity.

\subsection{Subject Winning Ratio ($\eta$)}
Rather than just considering the overall probability mass assigned to a subject, we also consider an alternative intuitive metric: \emph{How often does the model choose $x_1$ over it's counterpart?} This metric is more robust to large outlier values that could completely shift the probability mass in one direction. Additionally, we only consider ``wins'' beyond a specified threshold, $\theta$ to get the following \emph{winning ratio} metric:
%Although our winning score shows bias in probability mass across the dataset, idifferent score polarities might cancel each other out. Thus here we propose a complementary metric by counting how frequent winning scores are above certain threshold:
{
\begin{align}
    &\eta(x_1, \theta) = \frac{\displaystyle \sum_{\substack{\tau \in T, a\in A \\x_2 \in X}} \big[ \gamma(x_1|x_1, x_2, a) \geq \theta\big] }{|A|\times|T|\times|x_2|} \label{eq:naive_score}
\end{align}}
\daniel{should we use $\tau$ somewhere in the formula of $\gamma$?}
where $[\cdot]$ denotes indicator. As a result, an extremely stereo-typical model would have high scores in both $\gamma$ and $\eta$.

%\tushar{How can such a template be used to measure a bias? Remind them that we are looking at aggregate statistics based on these example-level measurements}
%\subsubsection{Question Answering}
%\tushar{Can be a small para on applying this template to QA model}
%\tushar{Can be a small para on applying this template to LMs}

==> [EMNLP'20] Unqovering Stereotypical Biases via Underspecified Questions/old_intro.tex <==

\section{Old Introduction}
Fine-tuning large, pre-trained language-models has been the dominant technical paradigm for building NLP models in the recent years~\cite{devlin-etal-2019-bert,liu2019roberta}. 
Such architectures learn representation of natural language from massive training corpus often drenched in stereotypical and biased statements~\cite{sun2019mitigating}.
% \ashish{`drenched in' claim needs a citation}. 
Not surprisingly, these problematic associations are picked up the pre-trained language-models and appear in the downstream tasks~\cite{kurita2019quantifying,tan2019assessing}.
\ashish{either mention which downstream tasks are covered in this prior work, or make a blanket statement that none of these covers QA.}

% In the recent pre-training and finetuning setting, neural representations are subject to further changes from the downstream datasets [cite] which also face such problem. 
% As a result, what we observe in a downstream QA model is unfair inferences as shown in Fig~\ref{fig:intro:example}.


% However, existing QA datasets do not suffice to show such biases since their examples are constructed to provide sufficient hint for an answer. On the other hand, well-specified hint could be a luxury in real-world application where models have to predict using their prior knowledge from time to time. In such scenario, a fair model is expected to yield predictions that comply with human common sense rather than to guess with stereotypical artifacts it picked up through the training process.

In this paper, we aim to use Question Answering (QA) as a high-level downstream task to uncover (and quantify) the biases within language models. 
\ashish{The above sentence begs the question: why? what's missing in prior work that this work seeks to address? I'm guessing people haven't studied stereotypical biases in QA models at all AND the bias detection mechanisms they have developed for their tasks either do not apply to QA or do not work adequately for QA. Is it true that probing different downstream tasks has been found to reveal different biases? If so, that would motivate looking at QA, in hopes of uncovering new / different degrees of biases than previously found. It's challenging to do this for QA (why?), so we introduce a new methodology (of using unspecified qns). Should address this first.}

\ashish{Save the mention of `templates', `fillers', etc., for later; that's about \emph{how} you do it. Start with a higher-level description of \emph{what}, just enough to understand the figure and why those questions are useful. E.g.: To probe for stereotypical bias for an action or attribute $A$ (e.g., being a bad driver) w.r.t.\ a sensitive attribute (e.g., gender, nationality), we design \emph{underspecified} questions, such as the ones shown in Fig.~\ref{fig:intro:example}. Each question describes a scenario with two individuals that differ in the sensitive attribute, and then asks who is the agent of $A$. By design, such a question is underspecified---there is no explicit evidence favoring either individual. A \emph{fair} model is thus expected to... .   [Also, separate out `in contrast to typical QA datasets' and its implications into a separate paragraph.]}
To this end, we design templates to produce questions that we will use to elicit the biases of the models. 
As shown in Fig~\ref{fig:intro:example}, 
the context of the questions describe a scenario involving  {\color{blue} a pair of fillers} ({\color{darkgreen} human names, nationalities, ethnicities, etc}). 
The questions ask about the agent of {\color{red} an action/attribute} --- often a negative one. 
% \daniel{underspecified defintion here}
Our questions, by design, are \emph{underspecified}, i.e., there is no explicit evidence favoring either of the fillers. 
This is in contrast with the typical definition of QA datasets, which are well-specified and constructed to provide sufficient hint for an, often, a unique answer. 
In our underspecified questions, a \emph{fair} model is expected to \emph{not} favor any of the subjects over the other ones. 
In contrast, assigning more likelihood to either of the subjects is an evidence for a biased inference. For instance, a model that considers more chance to an ``Asian'' person \ashish{`person' is good, but the example says `boy', and boys are too young to drive. change the example?} being ``a bad driver'' is violating the boundaries of ethical judgement by a blind association of a common stereotype --- the kind of biased judgement we want to avoid in natural language systems. 


% In this paper, we present a probe for such prior biases in QA model predictions. Our probe present underspecified QA examples where direct answer hints are omitted. As is shown in Fig~\ref{fig:intro:example}, instead of having totally unanswerable questions, we present two answer choices in each paragraph and models are free to make the best guess. Similar to [cite], we argue that the number of unfair inferences a model make depicts the degree of biases contained in the model.

% \daniel{association test and challenges}
% On the way to reveal stereotypical biases in QA models, we discover two other biases are actually dominant at the surface, i.e. positional bias and occurrence bias. We found that, without separating them, direct observation on probabilities of answer choices would lead to substantially different conclusions. This poses an extra challenge to designing bias metrics for QA models.

To be able to use underspecified question to quantify stereotypical biases \ashish{again same thing: before going into challenges, should make it clear \emph{why} you want to use underspecified questions in the first place. Is there an alternative people have tried? Does it not work well? Or is the proposal here the only natural choice?} in QA model, one has to overcome several challenges. 
In particular, other forms of biases in QA models, such as positional \ashish{worth a sentence / phrase to say what it is and even quantify it (by example) if it's a surprisingly large number!  E.g., we found that models tend to prefer agents mentioned closer to the action by as much as XX\%.} or occurrence biases, that dominate and skew their decision.  
One has to create a framework \ashish{let's see how it turns out; `framework' may be too big of a word, unless there is some support of generality of the method} to separate such compounding \emph{confounding?} factors to be able to focus on the biases that touch upon the ethical line (e.g., gender bias, nationality bias, etc). 
% Therefore, we propose a metric: Underspecified Comparative Association Test (UCAT) that peels off the two dominant biases and rank the degree of selectional biases over the two equally justifiable answers. For quantitative evaluation, we introduce \name, a dataset that is constructed by modifying natural sentences into underspecified ones, and use templates to augment them into millions of examples.
We propose a metric that peels off the two dominant biases \ashish{do we have evidence that these are `\textbf{the} two dominant biases'? to support this, we would want to quantitatively say these are dominant, not just two that we thought of and accounted for. This also touches upon the `exhaustive' aspect---are we saying there could be other ones, but they are not significant?} and rank the degree of selectional biases over the two equally justifiable answers.

For quantitative evaluation, we introduce a dataset that is constructed by modifying natural sentences into underspecified ones, and use templates \ashish{this is probably the first place you want to mention templates; not any earlier} to augment them into millions of examples.

\daniel{TODO: sth here about our exiciting results.}
\tao{Let's refer \name as the framework, not just the data neither just the metric}

%\daniel{do we need to use two keywords UCAT and UnQover? Or we can somehow merge them into one name?}

% To summarize, our contributions are:
% \begin{description}
%     \item 1: We introduce a bias probe for downstream QA models using underspecified examples.
%     \item 2: We present a metric UAT to evaluate model biases. And our experiments show that model predictions are subject to multiple biases, e.g. positional bias and availability bias.
% \end{description}

\paragraph{Contributions.}
We introduce a novel approach to probe biases in contextual language models by using \emph{underspecified} questions. \ashish{can we mention key benefits of this novel approach here? what does it enable / achieve that couldn't be done earlier?}
We introduce \textsc{UnQover}, a formal framework for quantifying biases based on underspecified questions. 
We show how this measure \ashish{measure?} helps neutralize other compounding factors like positional and occurrence bias that can interfere with the study of biases in our models.
This enables us to factor out these biases to get a true measure of gender, country and occupational biases in various QA models. 
We show that certain biases specifically are introduced by fine-tuning on the QA task, which were absent in the underlying language model.
Finally, upon publication we will release a \name\ leaderboard to quantify and compare the biased inferences of language models. 
To our knowledge, this is the first work that uses natural language questions to probe the biases in language-models. \ashish{This last sentence came a bit out of the blue. Better to introduce this aspect earlier, and also point out any benefits of this. This conflicts a bit with the mention of templates earlier, which generally point to synthetic language.}


==> old_equations_may20.tex <==
% \section{Reasoning Errors and Biases}
\section{Reasoning Errors of Question Answering Models and their Biases}
\label{sec:unintended_bias}
Before we go into the details of how we use our examples to detect biases, lets first consider \emph{what we can observe} as the output of our model and what \emph{we want to measure}. Given our generated examples and a QA model, we can measure the score assigned to a subject $x_1$ for the question based on $a$, represented as $\prob{x_1|\tau(x_1, x_2, a)}$ where $\tau(x_1, x_2, a)$ captures the (paragraph, question) pair generated by grounding our template $\tau$. For a QA model, these \daniel{simply} are \daniel{\sout{naturally}} probabilities of the span $x_1$ and $x_2$. 
\daniel{from this phrasing, is it clear that $\prob{x_1} + \prob{x_2} \neq 1$?}
For masked LM, we can use the probabilities for these subject tokens (assuming single-token subjects). However, what we want to measure is the stereotypical bias associated with $x_1$ compared to $x_2$ for $a$, represented as $\score{x_1| \{x_1, x_2, a\}}$.
%Note that the stereotypical bias score does \emph{not} depend on how the subjects and attributes are grounded by our template. \daniel{I don't understand this. Clarify this?}\tushar{actually this is not important in this formulation, so okay to drop.}

\daniel{
In $\score{x_1| \{x_1, x_2, a\}}$ notation, the use of set notation makes it seem like the ordering of $x_1, x_2, a$ does not matter, which is not the case. 
}

A natural approach to measure the bias, $\score{x_1| \{x_1, x_2, a\}} - \score{x_2| \{x_1, x_2, a\}}$ would be by directly comparing these predicted probabilities associated with the two subjects~\cite{de2019bias}, i.e., the bias of the model towards \slot{$x_1$} for activity \slot{$a$} could be measured as:
{
% \small
%\begin{equation}
\begin{align}
\score{x_1| \{x_1, x_2, a\}} - \score{x_2| \{x_1, x_2, a\}} = \nonumber\\
  \prob{x_1| \tau(x_1, x_2, a)} - \prob{x_2| \tau(x_1, x_2, a)}
\label{eqn:bias_score}
\end{align}
%\end{equation}
}
However, models sometimes focus on artifacts in the input leading to inconsistent behaviors. For example, $\score{x_1| \{x_1, x_2, a\}}$ does not depend on the ordering of $x_1$ and $x_2$, i.e.  $\score{x_1| \{x_1, x_2, a\}}=\score{x_1| \{x_2, x_1, a\}}$, but this is not the case with a RoBERTa SQuAD model:
%\emph{[An example with extreme probabilities and inconsistent predictions]}
\egbox{
    
    {\small Paragraph: The person over the swing is \sfiller{Justin}. Sitting by the side is \sfiller{Alice}.}\\
    {\small Question: Who \afiller{was a bodyguard}? }\\ 
    \text{   } {\small $\prob{\sfiller{Alice}}\texttt{=}0.77$ \hspace{2ex} $\prob{\sfiller{Justin}}\texttt{=}0.21$.} \\
    \\
    {\small Paragraph: The person over the swing is \sfiller{Alice}. Sitting by the side is \sfiller{Justin}.}\\
    {\small Question: Who \afiller{was a bodyguard}? }\\ 
    \text{   } {\small $\prob{\sfiller{Alice}}\texttt{=}0.03$ \hspace{2ex} $\prob{\sfiller{Justin}}\texttt{=}0.96$.}
    }
where predictions are completely changed by just swapping the subjects positions, even though the information in the context is effectively the same.
%\tushar{Can we change the example with a more symmetric context? Arguably bodyguards are never the ones on swings :)}



%In this paper, we aim to measure stereotypical biases via underspecified questions. That is, with both subjects are equally justifiable for a question, model should predict fair distribution over them. Unfair predictions can be attributed to biases, known or unknown, and reasoning errors. When measuring stereotypical biases, we expect a metric to be as robust as possible against errors and variances such that there is no false positive.

%In this section, we present our discoveries on two major categories of reasoning errors that exist in both QA and pre-trained language models: \textbf{position inconsistency} and \textbf{negation inconsistency}. We argue that a robust evaluation has to peel off the effect of such reasoning errors, otherwise one might end up with contradicting observations.

Furthermore, models might not always capture what the question is intended to ask:
%While our bias score is position invariant, it should be highly dependent on the attribute in the question. However, models may not always capture the question accurately, e.g., the RoBERTa SQuAD model has roughly the same scores for two questions with exactly opposite meaning!
%consider the example predictions from a RoBERTa SQuAD model:
%\emph{[An example with extreme probabilities and inconsistent predictions]}
\egbox{
    {\small Paragraph: The person over the swing is \sfiller{Justin}. Sitting by the side is \sfiller{Alice}.}\\
    {\small Question: Who \afiller{was a bodyguard}? }\\ 
    \text{   } {\small $\prob{\sfiller{Alice}}\texttt{=}0.77$ \hspace{2ex} $\prob{\sfiller{Justin}}\texttt{=}0.21$.} \\
    {\small Question: Who \afiller{can never be a bodyguard}?} \\
    \text{   } {\small $\prob{\sfiller{Alice}}\texttt{=}0.87$ \hspace{2ex} $\prob{\sfiller{Justin}}\texttt{=}0.10$.}
}

\emph{Given these reasoning errors\footnote{We call them reasoning errors since a robust model should not be affected by such meaning invariant changes (and should be affected by the change in question meaning).}, how can we accurately capture the stereotypical biases of QA models?} We will show how these issues can be isolated to reveal the true stereotypical bias in the model. 

\subsection{Decomposing Reasoning Errors and Biases}
While the stereotypical bias $\score{x_1| \{x_1, x_2, a\}}$ is based on all of its inputs, the model scores could be affected by artifacts based on partial inputs. We capture this as a linear combination of the bias term with all possible partial interactions that are not indicative of this bias:
\begin{align}
    %\forall \tau, \prob{x_1| \tau(x_1, x_2, a)} =  \score{x_1| \{x_1, x_2, a\}} + \nonumber\\
    %f(x_1, x_2, \tau) + g(\{x_1, x_2\}, a) \label{eqn:components}
    \forall \tau, &\; \prob{x_1| \tau(x_1, x_2, a)} =  \score{x_1| \{x_1, x_2, a\}} + \nonumber\\
    & f(x_1| x_2, \tau) + g(x_1 |x_2, a) \label{eqn:components}
\end{align}
%We basically assume that the model's score is a linear combination of a robust score based on all the inputs (i.e. the bias) and all possible partial interactions within $\{x_1, x_2, a\}$ that would not capture the bias.
where the first component $f(x_1 | x_2, \tau)$ captures the models' preference purely based on the paragraph irrespective of the attribute; the second component $g(x_1 | x_2, a)$ captures the model's preference purely based on lexical cues in the attribute irrespective of the subject ordering and sentence structure in $\tau$.\tushar{We shouldn't have "a" in g. The point is that g is the factor that does not depend on a. So it would stay the same for both a and $\bar{a}$. I see the value of $x_1|x_2$ in g as it makes it clear that the bias is towards $x_1$ but it also makes it seem order-dependent.}
%Note that model's decisions to choose any subject purely based on the question would still fall under the umbrella of bias. For simplicity, we ignore terms purely based on $a$ as they would appear in $\prob{x_2| \tau(x_1, x_2, a)}$ too and cancel each other out. 
%Henceforth, we will only model $g(x_1)$ and assume $h(x_2)$ would be captured by $\prob{x_2| \tau(x_1, x_2, a)}$.

Our goal here is to isolate the components $f$ and $g$ for the a given template $\tau$. To isolate $f$, we will use subject-symmetric examples $\tau(x_1, x_2, a)$ and $\tau(x_2, x_1, a)$ where the only variant for the model to make different predictions would be the subject position. We will refer this to \emph{positional artifact} in Sec~\ref{subsec:position_bias}.
For component $g$, we will use polarized attributes\tushar{What are polarized attributes?} where models rely on lexical cues in the attribute to make predictions. We will refer this to \emph{attributive artifact} in Sec~\ref{subsec:preference_bias}.


%The first term:  $f(x_1, x_2, \tau)$ captures the score purely based on the paragraph. For symmetric templates, the information captured by $\tau(x_1, x_2, a)$ should be exactly same as $\tau(x_2, x_1, a)$. \tao{dont want to say exactly.} So the only phenomenon that the model relies on to make different predictions for $\tau(x_1, x_2, a)$ vs $\tau(x_2, x_1, a)$ would be the position of these subjects. Note that even if the template is not symmetric, our solution to factor out the term $f(x_1, x_2, \tau)$ would correct any position-specific bias introduced by our templates. \tao{the last sent is too detailed.}


%The second term: $g({x_1, x_2}, \tau)$ captures the model's relative preference toward a particular subject irrespective of order and the attribute in the question. It may also be relying on lexical cues from the template, but importantly does not rely on the input attribute. The influence of this term can be seen in the example above, where changing the question had minimal effect due to the dominant effect of this score. 

Since these are the only possible terms that do not capture bias, if we factor these terms out, we will be left with only the sterotypical bias of the model. We will focus on isolating these reasoning errors individually first and then combine them to derive our final score.

%So can we say the model is actually fair because some reasoning errors overwrite stereotypical biases (if there is any)? We will show the asnwer is \emph{no}. After peeling off errors in model predictions, stereotypical biases are revealed.


\subsection{Positional Artifacts($\mu$)}
\label{subsec:position_bias}
As shown above, flipping subject positions would change model predictions.
But this shouldn't change the bias score.
By measuring this shift in model scores between the two orderings, we can measure this error:
%\tao{Doing simplification}
%As we show above, certain models have an implicit tendency to pick one subject over another purely based on its position in text. In such a case, flipping the subject positions would change the model predictions, but shouldn't change the bias score.  
%In such a case, flipping the answer positions would also flip model predictions. This \emph{flip} in model predictions can be measured by comparing the shift in probability between the two subject orderings. Specifically we can measure this type of error on the \emph{second} subject as:
{
\begin{align*}
    \mu(x_1, x_2, a) = \prob{x_1| \bar{\tau}(a)} \texttt{-} \prob{x_1| \tau(a)}
\end{align*}
}
where $\tau(a)$ denotes the subject-instantiated example $\tau(x_1, x_2, a)$ and the flipped version $\bar{\tau}(a)=\tau(x_2,x_1,a)$\footnote{We will assume there is only one template $\tau$ to simplify notation. In practice, we use multiple templates.}.
Given our definition in Eq~\ref{eqn:components}, 
%$\prob{x_1| \tau(x_1, x_2, a)} =  \score{x_1| \{x_1, x_2, a\}} + f(x_1, x_2, \tau)$, 
this score captures the relative bias between the two positions, i.e.
\begin{align*}
        \mu(x_1, x_2, a) = f(x_1 | x_2, \tau) - f(x_1 | x_2, \bar{\tau})
\end{align*}


We can also measure this value for our entire dataset by aggregating this value across all the examples, i.e.,
{
\begin{equation}
    \label{eq:pos_score}
    \mu = \frac{\sum_{
        \substack{
            x_1\in X_1 \\ 
            x_2\in X_2 \\ 
            a \in A
        }
    } \mu(x_1, x_2, a) }{|X_1| \times |X_2|\times|A|},
\end{equation}
}
where $X_1$ and $X_2$ are the set of subjects and $A$ are the set of attributes. $\mu$ falls in range $[-1,+1]$ and would be zero for a model with no position bias. 

\paragraph{Isolating Positional Artifacts.} 
While we can not directly measure $f$, by averaging the model's scores for both positions, we can factor them out in our comparative bias computation, i.e., we compute the position-invariant score for $x_1$ as
%When measuring the true stereotypical bias, we need to factor out this inconsistency. To do so, we include both orderings of subjects in our example and average the two probabilities to get the model's preference towards a particular subject. The position-corrected score for subject $x_1$ would be:
%We will introduce our metric in Section~\ref{sec:metric}
% \tushar{This is different though, right? It is talking about what it would mean to only isolate position bias and I am hoping gives intuition about the final metric.}

\begin{align*}
  &s_{\mu}(x_1| a) \texttt{=} \frac{1}{2}\Big[\prob{x_1| \tau(a)} \texttt{+}  \prob{x_1| \bar{\tau}(a)}\Big] \\
   &\hspace{2ex}\texttt{=}\score{x_1| \{x_1, x_2, a\}} \texttt{+} g(x_1|x_2,a) \texttt{+} \\
   & \hspace{3ex} \frac{1}{2}\Big[ f(x_1|x_2,\tau) \texttt{+} f(x_1|x_2,\bar{\tau})\Big]
  %=& \score{x_1| \{x_1, x_2, a\}} + \frac{1}{2}\Big[ f(\tau) + f(\bar{\tau})\Big]
\end{align*}
In the running example, when the activity $a$=\afiller{was a bodyguard}, we have $s_\mu(\sfiller{Alice})=0.4$ and $s_\mu(\sfiller{Justin})=0.59$.

%\tao{We are not done yet. Too early to jump to the below conclusion.}
%i.e. the model was actually biased towards \sfiller{Justin} being the \afiller{bodyguard}. Also note that the latter term would be exactly same for $\score{x_2| \{x_1, x_2, a\}}$ and so the final comparative bias based on this score would capture the true stereotypical bias:
%\begin{align*}
%&s_{\mu}(x_1| \tau(a))  -  s_{\mu}(x_2| \tau(a)) = \\
%& \hspace{1ex} \score{x_1| \{x_1, x_2, a\}}  - \score{x_2| \{x_1, x_2, a\}} + \\
%& \hspace{1ex} g(x_1|x_2,a) - g(x_2|x_1,a)
%\end{align*}
%where we assume position has a linear component in model predictions.



%Similar score can be computed for \slot{$x_2$} and then compared to $ \text{score}(x_1| x_2, a)$ to get the model's bias. Note that for a model with no position bias, i.e $\mu_2(x_1, x_2, a) = 0$, these two probabilities would be exactly same and map to the model's predicted probability.
%In our underspecified setting, we consider position bias as how much a subject's position is preferred over the other position. We measure it by the averaged winning score of the first subject over the second subject over all examples and questions. We denote it by $\mu(1st)$, and $\mu(2nd)=-\mu(1st)$.

%\tushar{TODO: Add simple example to map this equation to a real example}

\subsection{Attributive Artifacts ($\nu$)}
\label{subsec:preference_bias}
%But is it true even if the question is negated?
% We have seen that, in the above example, sometimes models seem do not understand the question.
%This kind of inconsistency is very hard to detect as it would appear very similar to the stereotypical bias in the model. For example, if the model is biased towards a particular subject for all activities in our set, it would also appear as a preference bias.
%To measure such errors, we need to introduce alternate activities that would change the prediction of the stereotypical bias model. but not the model with preference bias. Specifically, for every activity in our set $a$, we introduce a negated activity $\bar{a}$ such that a stereo-typical model, that chooses $x_1$ as the answer for $a$, would \emph{not} choose it be the answer for $\bar{a}$, i.e. anti-stereotypical. For example, for the activity: $a$=\afiller{is a country full of poor people}, we create a negated activity: $\bar{a}$ = \afiller{is a country full of rich people}. 
Unlike positional artifact, we expect the bias score to change with the attribute. But as we observe, this may not be the case in our QA models. So to measure this error, we need to introduce an attribute that should, by design, change the model prediction and then measure the model's invariance.

%Specifically, we use a negated attribute $\bar{a}$ for each $a$ such that a stereotypical model, that chooses $x_1$ as the answer for $a$, would ideally not choose it for $\bar{a}$.

For subject $x_1$, we can measure this error based on the change in probabilities over the polarized pair $(a,\bar{a})$:
%At each instance level, we can compare the scores across two polarized activities: $P(x_1| \tau(x_1, x_2, a))$ and $P(x_1| \tau(x_1, x_2, \bar{a}))$ which when aggregated across the examples gives us the preference bias of the model:
{
\begin{align}
    \nu(x_1, x_2, a) & = 1 \texttt{-} \Big| \prob{x_1| \tau(a)} \texttt{-} \prob{x_1| \tau(\bar{a})} \Big|  \nonumber 
\end{align}

\begin{align}
    \nu = \frac{\sum_{x_1 \in X_1, x_2 \in X, a \in A} \nu(x_1, x_2, a)}{|{X_1}|\times|{X_2}|\times|A|},
        \label{eq:pref_score}
\end{align}
}
where $\tau(\bar{a})=\tau(x_1,x_2,\bar{a})$. 
%Note that a model, that blindly prefers a particular answer irrespective of the activity, would not have much change in predictions.
Note that when the model ignores the semantics of attribute $a$, it would have $g(x_1| x_2, a)=g(x_1|x_2,\bar{a})$ resulting in $\nu=1$, whereas any difference in probabilities would reduce this score.
% Specifically given $\prob{x_1| \tau(x_1, x_2, a)} =  \score{x_1| \{x_1, x_2, a\}} + g(\{x_1, x_2\}, \tau)$, this term captures $\nu(x_1, x_2, a) = 1 - |\score{x_1| \{x_1, x_2, a\}} - \score{x_1| \{x_1, x_2, \bar{a}\}}|$.
%Note that lack of stereotype is also a form of attribute invariance, which would appear as $\nu=0$. 
%\tushar{This might be a better metric: higher implies more bias and change in signs doesn't cancel things out.} 
%\tushar{Both this metric and our previous metric has another problem: Lack of stereotypical bias would appear as preference bias.}

\paragraph{Isolating Attribute Invariance} To factor out this error, we adopt a similar approach as in Section~\ref{subsec:position_bias}, i.e. to include both polarized activities in our example. But unlike positional artifacts, we want to measure the relative change, captured by the difference between the two scores:
%Our metric in Section~\ref{sec:metric} will score each example based on the relative preference of an activity over its negated counterpart.
\begin{align*}
  & s_{\nu}(x_1|\tau(a)) \texttt{=} \frac{1}{2}\Big[\prob{x_1| \tau(a)} \texttt{-} \prob{x_1| \tau(\bar{a})}\Big] \\
  %& \hspace{2ex} \textt{=} 
\end{align*}
In the running example, we have $s_\nu(\sfiller{Alice})=-0.05$ and $s_\nu(\sfiller{Justin})=0.05$.

This metric would automatically factor out the attribute invariant term: $g(\{x_1, x_2\}, \tau)$. Moreover, if we assume that $\score{x_1| \{x_1, x_2, \bar{a}\}}$ = $C - \score{x_1| \{x_1, x_2, a\}}$, for some constant C, this metric will give us the exact bias score shifted by a constant term:
\begin{align}
    s_{\nu}(x_1|\tau(a)) =  &\frac{1}{2}\Big[\score{x_1| \{x_1, x_2, a\}} - \nonumber\\
    & \hspace{0.5cm} \score{x_1| \{x_1, x_2, \bar{a}\}}\Big] \nonumber\\
     = &\score{x_1| \{x_1, x_2, a\}} - \frac{C}{2}
     \label{eq:pref_fix}
\end{align}
and the difference $s_{\nu}(x_1|\tau(a))-s_{\nu}(x_2|\tau(a))$ exactly captures the comparative stereotypical bias.
%And the difference $s_{\nu}(x_1|\tau(a)) & - s_{\nu}(x_2|\tau(a))$ would accurately capture the true score:
 %    \score{x_1| \{x_1, x_2, a\}}& - \score{x_2| \{x_1, x_2, a\}}$
In the next section, we will present our final metric to compute stereotypical bias based on these two metrics.
%\tushar{TODO: Add the underlying linear combination assumption. Also add the caveat for what happens when $a=\bar{a}$ for a model}

%\tushar{Should we halve this?}
%In such a case, flipping the order of the subjects would also flip the answer selected by our model. This \emph{flip} in model predictions can be measured by comparing the shift in probability between the two subject orderings. Specifically we can measure the bias towards the second subject as, i.e.
% At instance level, we consider preference bias as how much the probability changes on a particular subject when the question activity is negated. We measure this in absolute scale:
% {\small
% \begin{align}
%     \nu(t, \alpha) =& \frac{1}{2} \big(| P(x_1|t,a)-P(x_1|t,\bar{a}) | \nonumber \\
%     & +|P(x_2|t,a) - P(x_2|t,\bar{a})| \big)
%     \label{eq:pos_score}
% \end{align}
% }
% and at dataset level, we take the average over example $t$'s and activity pair $\alpha$'s. Ideally, a model predicts drastically different probabilities on the negated activity pair $\alpha$, such that $\nu=1$.

\section{Uncovering Stereotypical Biases} \label{sec:metric}
In this section, we will combine our mitigation tactics to define our final sterotypical bias score for any example. We then present two metrics to aggregate these scores across examples.

\subsection{Example Bias Score}
Lets consider Equation~\ref{eqn:components} with both the confounding factors. While each of our individual proposed scores only handle one of these factors, a simple combination of these scores cancel both of the factors out. Specifically, a simple combination of ideas from $s_\mu$ and $s_\nu$ leads to a metric that captures only the stereotypical bias score:
{\small
\begin{align}
    \gamma(x_1| x_1, x_2, a) \texttt{=} & \frac{1}{2} \Big[ s_\mu(x_1|\tau(a)) \texttt{-} s_\mu(x_1|\tau(\bar{a})) \nonumber\\
    & \texttt{-} \big[ s_\mu(x_2|\tau(a)) \texttt{-} s_\mu(x_2|\tau(\bar{a})) \big] \Big] \nonumber
\end{align}}
where $s_\mu(x_1|\tau(a)) \texttt{-} s_\mu(x_1|\tau(\bar{a}))$ captures the position-adjusted (within $s_\mu$) and attribute-adjusted (through the difference between $a$ and $\bar{a}$) score for $x_1$. The first half can be shown to simplify to the exact same term as Equation~\ref{eq:pref_fix}
{\small
\begin{align}
   & s_\mu(x_1|\tau(a)) \texttt{-} s_\mu(x_1|\tau(\bar{a}) \nonumber \\
   &=  \score{x_1| \{x_1, x_2, a\}} + \frac{1}{2}\big[ f(\tau) + f(\bar{\tau})\big] + g(\{x_1, x_2\}, \tau) \nonumber\\
   & -  \Big[\score{x_1| \{x_1, x_2, \bar{a}\}} + \frac{1}{2}\big[ f(\tau) + f(\bar{\tau})\big] + g(\{x_1, x_2\}, \tau)\Big] \nonumber\\
   & =  \score{x_1| \{x_1, x_2, a\}} - C/2 \nonumber
\end{align}}
We can prove a similar result for the second half leading to the difference between the terms capturing the true sterotypical bias:
{\small
\begin{align*}
    \gamma(x_1| x_1, x_2, a) \texttt{=} \score{x_1| \{x_1, x_2, a\}} - \score{x_2| \{x_1, x_2, a\}}
\end{align*}
}
An alternate equivalent formulation can also be similarly proven to capture the true bias:
{\small
\begin{align}
    \gamma(x_1| x_1, x_2, a) \texttt{=} & \frac{1}{2} \Big[ s_\nu(x_1|\tau(a)) \textt{+} s_\nu(x_1|\bar{\tau}(a)) \nonumber\\
    & \texttt{-} \big[s_\nu(x_2|\tau(a)) \textt{+} s_\nu(x_2|\bar{\tau}(a)) \big] \Big]
\end{align}}
where  $s_\nu(x_1|\tau(a)) \texttt{+} s_\nu(x_1|\bar{\tau}(a)))$ captures the position-adjusted (through the averaging across $\tau$ and $\bar{\tau}$) and attribute-adjusted (within $s_\mu$) score for $x_1$
\tushar{Tao: Does the above look correct?}


Consider the four example questions created through a single template in Figure~\ref{fig:example}. In essence, we first compute the position adjusted score by summing the scores for the two different orders in each row. We then subtract the bottom scores from the top to get the true stereotypical score for each $x_1$ and $x_2$. \tushar{Very hand-way. should we add the exact computation?}

We next present our two aggregate metrics that capture the models bias towards \textbf{one} subject relative to all others. 

\subsection{Subject Bias Score}

% By directly comparing two subjects in our examples, the degree of bias is naturally reflect by how much a subject is preferred over another. We argue that such comparison must be made after peeling off the effect of position and preference inconsistencies. For how much subject $x_1$ wins over $x_2$:

% {\small
% \begin{align}
%     & \gamma(x_1| x_1, x_2, a) \\ 
%     & \texttt{=} \frac{1}{2} \big[ s_\mu(x_1|\tau(a)) \texttt{-} s_\mu(x_1|\tau(\bar{a})) \texttt{+} s_\mu(x_2|\tau(\bar{a})) \texttt{-} s_\mu(x_2|\tau(a)) \big] \nonumber \\
%     & \texttt{=} \frac{1}{2} \big[ s_\nu(x_1|\tau(a)) \textt{+} s_\nu(x_1|\bar{\tau}(a)) \texttt{-} s_\nu(x_2|\tau(a)) \textt{-} s_\nu(x_2|\bar{\tau}(a)) \big] \nonumber
% \end{align}}
% \daniel{in the 2nd line, the bars should on on a's not tau's?}
% \daniel{also, I am not sure if you actually need the 2nd line}
% That is, the probability difference $\gamma$ is computed by subtracting the position-independent and negation-independent score of $x_2$ from that of $x_1$.


\begin{figure*}
    \centering
    % you can update the figure here: https://www.draw.io/#G1I9uZ2Ts7s6ygpOoqUdjbzQGA88al4-Q- 
    \includegraphics[scale=0.71]{figures/example-2.pdf}
    \caption{TODO}
    \label{fig:example}
\end{figure*}

% \tushar{TODO An example with all four instantiations of one template}
% \daniel{added an example to figure: Figure~\ref{fig:example}; some numbers are missing but see if the general structure looks good. }
%Our per-example stereotypical bias score $\gamma$ represents how probabilities are massed towards one subject over the other. 
Since these measurements can be volatile per-example\tushar{This seems a bit backward. We designed our approach with this issue in mind and not just designing the solution now. Rather we should say that we use our per-example score to capture the subject-level bias via aggregation.}, we aggregate them across examples to capture the model bias on subject $x_1$: 

{
\begin{align}
    & \gamma(x_1) = \frac{\displaystyle \sum_{\substack{\tau \in T, a\in A \\ x_2 \in X}} \gamma(x_1| x_1, x_2, a) }{|A|\times|T|\times|x_2|}
\end{align}
\daniel{should we use $\tau$ somewhere inside the parenthesis of $\gamma$?}
}
where $X$ denotes the set of subjects, $T$ the set of templates, $A$ the set of activities.
Ideally, a fair model would have $\gamma=0$. Having positive $\gamma$ indicates subject $x_1$ is biased towards the activity, and negative score represents the subject is biased away from the activity.

\subsection{Subject Winning Ratio ($\eta$)}
Rather than just considering the overall probability mass assigned to a subject, we also consider an alternative intuitive metric: \emph{How often does the model choose $x_1$ over it's counterpart?} This metric is more robust to large outlier values that could completely shift the probability mass in one direction. Additionally, we only consider ``wins'' beyond a specified threshold, $\theta$ to get the following \emph{winning ratio} metric:
%Although our winning score shows bias in probability mass across the dataset, idifferent score polarities might cancel each other out. Thus here we propose a complementary metric by counting how frequent winning scores are above certain threshold:
{
\begin{align}
    &\eta(x_1, \theta) = \frac{\displaystyle \sum_{\substack{\tau \in T, a\in A \\x_2 \in X}} \big[ \gamma(x_1|x_1, x_2, a) \geq \theta\big] }{|A|\times|T|\times|x_2|} \label{eq:naive_score}
\end{align}}
\daniel{should we use $\tau$ somewhere in the formula of $\gamma$?}
where $[\cdot]$ denotes indicator. As a result, an extremely stereo-typical model would have high scores in both $\gamma$ and $\eta$.

%\tushar{How can such a template be used to measure a bias? Remind them that we are looking at aggregate statistics based on these example-level measurements}
%\subsubsection{Question Answering}
%\tushar{Can be a small para on applying this template to QA model}
%\tushar{Can be a small para on applying this template to LMs}

==> old_intro.tex <==

\section{Old Introduction}
Fine-tuning large, pre-trained language-models has been the dominant technical paradigm for building NLP models in the recent years~\cite{devlin-etal-2019-bert,liu2019roberta}. 
Such architectures learn representation of natural language from massive training corpus often drenched in stereotypical and biased statements~\cite{sun2019mitigating}.
% \ashish{`drenched in' claim needs a citation}. 
Not surprisingly, these problematic associations are picked up the pre-trained language-models and appear in the downstream tasks~\cite{kurita2019quantifying,tan2019assessing}.
\ashish{either mention which downstream tasks are covered in this prior work, or make a blanket statement that none of these covers QA.}

% In the recent pre-training and finetuning setting, neural representations are subject to further changes from the downstream datasets [cite] which also face such problem. 
% As a result, what we observe in a downstream QA model is unfair inferences as shown in Fig~\ref{fig:intro:example}.


% However, existing QA datasets do not suffice to show such biases since their examples are constructed to provide sufficient hint for an answer. On the other hand, well-specified hint could be a luxury in real-world application where models have to predict using their prior knowledge from time to time. In such scenario, a fair model is expected to yield predictions that comply with human common sense rather than to guess with stereotypical artifacts it picked up through the training process.

In this paper, we aim to use Question Answering (QA) as a high-level downstream task to uncover (and quantify) the biases within language models. 
\ashish{The above sentence begs the question: why? what's missing in prior work that this work seeks to address? I'm guessing people haven't studied stereotypical biases in QA models at all AND the bias detection mechanisms they have developed for their tasks either do not apply to QA or do not work adequately for QA. Is it true that probing different downstream tasks has been found to reveal different biases? If so, that would motivate looking at QA, in hopes of uncovering new / different degrees of biases than previously found. It's challenging to do this for QA (why?), so we introduce a new methodology (of using unspecified qns). Should address this first.}

\ashish{Save the mention of `templates', `fillers', etc., for later; that's about \emph{how} you do it. Start with a higher-level description of \emph{what}, just enough to understand the figure and why those questions are useful. E.g.: To probe for stereotypical bias for an action or attribute $A$ (e.g., being a bad driver) w.r.t.\ a sensitive attribute (e.g., gender, nationality), we design \emph{underspecified} questions, such as the ones shown in Fig.~\ref{fig:intro:example}. Each question describes a scenario with two individuals that differ in the sensitive attribute, and then asks who is the agent of $A$. By design, such a question is underspecified---there is no explicit evidence favoring either individual. A \emph{fair} model is thus expected to... .   [Also, separate out `in contrast to typical QA datasets' and its implications into a separate paragraph.]}
To this end, we design templates to produce questions that we will use to elicit the biases of the models. 
As shown in Fig~\ref{fig:intro:example}, 
the context of the questions describe a scenario involving  {\color{blue} a pair of fillers} ({\color{darkgreen} human names, nationalities, ethnicities, etc}). 
The questions ask about the agent of {\color{red} an action/attribute} --- often a negative one. 
% \daniel{underspecified defintion here}
Our questions, by design, are \emph{underspecified}, i.e., there is no explicit evidence favoring either of the fillers. 
This is in contrast with the typical definition of QA datasets, which are well-specified and constructed to provide sufficient hint for an, often, a unique answer. 
In our underspecified questions, a \emph{fair} model is expected to \emph{not} favor any of the subjects over the other ones. 
In contrast, assigning more likelihood to either of the subjects is an evidence for a biased inference. For instance, a model that considers more chance to an ``Asian'' person \ashish{`person' is good, but the example says `boy', and boys are too young to drive. change the example?} being ``a bad driver'' is violating the boundaries of ethical judgement by a blind association of a common stereotype --- the kind of biased judgement we want to avoid in natural language systems. 


% In this paper, we present a probe for such prior biases in QA model predictions. Our probe present underspecified QA examples where direct answer hints are omitted. As is shown in Fig~\ref{fig:intro:example}, instead of having totally unanswerable questions, we present two answer choices in each paragraph and models are free to make the best guess. Similar to [cite], we argue that the number of unfair inferences a model make depicts the degree of biases contained in the model.

% \daniel{association test and challenges}
% On the way to reveal stereotypical biases in QA models, we discover two other biases are actually dominant at the surface, i.e. positional bias and occurrence bias. We found that, without separating them, direct observation on probabilities of answer choices would lead to substantially different conclusions. This poses an extra challenge to designing bias metrics for QA models.

To be able to use underspecified question to quantify stereotypical biases \ashish{again same thing: before going into challenges, should make it clear \emph{why} you want to use underspecified questions in the first place. Is there an alternative people have tried? Does it not work well? Or is the proposal here the only natural choice?} in QA model, one has to overcome several challenges. 
In particular, other forms of biases in QA models, such as positional \ashish{worth a sentence / phrase to say what it is and even quantify it (by example) if it's a surprisingly large number!  E.g., we found that models tend to prefer agents mentioned closer to the action by as much as XX\%.} or occurrence biases, that dominate and skew their decision.  
One has to create a framework \ashish{let's see how it turns out; `framework' may be too big of a word, unless there is some support of generality of the method} to separate such compounding \emph{confounding?} factors to be able to focus on the biases that touch upon the ethical line (e.g., gender bias, nationality bias, etc). 
% Therefore, we propose a metric: Underspecified Comparative Association Test (UCAT) that peels off the two dominant biases and rank the degree of selectional biases over the two equally justifiable answers. For quantitative evaluation, we introduce \name, a dataset that is constructed by modifying natural sentences into underspecified ones, and use templates to augment them into millions of examples.
We propose a metric that peels off the two dominant biases \ashish{do we have evidence that these are `\textbf{the} two dominant biases'? to support this, we would want to quantitatively say these are dominant, not just two that we thought of and accounted for. This also touches upon the `exhaustive' aspect---are we saying there could be other ones, but they are not significant?} and rank the degree of selectional biases over the two equally justifiable answers.

For quantitative evaluation, we introduce a dataset that is constructed by modifying natural sentences into underspecified ones, and use templates \ashish{this is probably the first place you want to mention templates; not any earlier} to augment them into millions of examples.

\daniel{TODO: sth here about our exiciting results.}
\tao{Let's refer \name as the framework, not just the data neither just the metric}

%\daniel{do we need to use two keywords UCAT and UnQover? Or we can somehow merge them into one name?}

% To summarize, our contributions are:
% \begin{description}
%     \item 1: We introduce a bias probe for downstream QA models using underspecified examples.
%     \item 2: We present a metric UAT to evaluate model biases. And our experiments show that model predictions are subject to multiple biases, e.g. positional bias and availability bias.
% \end{description}

\paragraph{Contributions.}
We introduce a novel approach to probe biases in contextual language models by using \emph{underspecified} questions. \ashish{can we mention key benefits of this novel approach here? what does it enable / achieve that couldn't be done earlier?}
We introduce \textsc{UnQover}, a formal framework for quantifying biases based on underspecified questions. 
We show how this measure \ashish{measure?} helps neutralize other compounding factors like positional and occurrence bias that can interfere with the study of biases in our models.
This enables us to factor out these biases to get a true measure of gender, country and occupational biases in various QA models. 
We show that certain biases specifically are introduced by fine-tuning on the QA task, which were absent in the underlying language model.
Finally, upon publication we will release a \name\ leaderboard to quantify and compare the biased inferences of language models. 
To our knowledge, this is the first work that uses natural language questions to probe the biases in language-models. \ashish{This last sentence came a bit out of the blue. Better to introduce this aspect earlier, and also point out any benefits of this. This conflicts a bit with the mention of templates earlier, which generally point to synthetic language.}

